Equality Constrained Linear Optimal Control With Factor Graphs

This paper presents a novel factor graph-based approach to solve the discrete-time finite-horizon Linear Quadratic Regulator problem subject to auxiliary linear equality constraints within and across time steps. We represent such optimal control problems using constrained factor graphs and optimize the factor graphs to obtain the optimal trajectory and the feedback control policies using the variable elimination algorithm with a modified Gram-Schmidt process. We prove that our approach has the same order of computational complexity as the state-of-the-art dynamic programming approach. Furthermore, current dynamic programming approaches can only handle equality constraints between variables at the same time step, but ours can handle equality constraints among any combination of variables at any time step while maintaining linear complexity with respect to trajectory length. Our approach can be used to efficiently generate trajectories and feedback control policies to achieve periodic motion or repetitive manipulation.

==> sections/sec_appedix.tex <==
We provide a probabilistic view of Figure \ref{fig:lqr_suba} to show the essence of factor graphs. If we treat $X = [x_2; u_1; x_1; u_0; x_0]$ as a stack of random variables, before connecting variables with edges it has a prior distribution $p(X)$. We then define three types of likelihood functions \cite{dong2016motion}:
\begin{align}
  l_{objx} (x_t; \mathcal{Q}_t) & \propto P(\mathcal{Q}_t|x_t)  = \exp \Big\{ -\frac{1}{2}\| x_t \|^2_{Q_{xx_t}}    \Big\}, \label{eqn:likelihood_x}\\
   l_{obju} (u_t; \mathcal{R}_t) &  \propto P(\mathcal{R}_t|u_t)  = \exp \Big\{ -\frac{1}{2}\| u_t \|^2_{Q_{uu_t}}    \Big\},  \label{eqn:likelihood_u}\\
   l_{dyn} (x_{t+1}, x_t, u_t; \mathcal{F}_t) & \propto P(\mathcal{F}_t|x_{t+1}, x_t, u_t) \nonumber \\    = &\exp \Big\{ -\frac{1}{2}\| x_{t+1} - F_{x_t}x_t + F_{u_t}u_t  \|^2_{\Sigma_c}    \Big\},\label{eqn:likelihood_cst}
\end{align}
where $\|\cdot\|_{\Sigma}$ is the Mahalanobis norm, and $\Sigma$ is the covariance of the distribution. Notice $\Sigma_c \to 0$. As the definition suggests, a likelihood function measures the probability of elements in the random variable $X$ on condition that a ``factor event'' such as $\mathcal{Q}$ be 0. It's not hard to see the correspondences between edges in Figure \ref{fig:lqr_suba} and likelihood functions. Define all factor events as $Z=[\mathcal{F}_1,\mathcal{F}_2,\mathcal{Q}_0,\mathcal{Q}_1,\mathcal{Q}_2,
\mathcal{R}_0,\mathcal{R}_1]$, the joint probability distribution of $X$ and $Z$ is essentially
\begin{align}
p(X,Z) = & p(Z|X)p(X) \nonumber \\ 
= & p(x_0,u_0,x_1,u_1,x_2,
\mathcal{F}_1,\mathcal{F}_2,\mathcal{Q}_0,\mathcal{Q}_1,\mathcal{Q}_2,
\mathcal{R}_0,\mathcal{R}_1) \nonumber\\
= & p(\mathcal{Q}_0|x_0)p(\mathcal{Q}_1|x_1) p(\mathcal{F}_1|x_0,u_0,x_1)p(\mathcal{F}_2|x_1,u_1,x_2) \nonumber \\
  & p(\mathcal{R}_0|u_0)p(\mathcal{R}_1|u_1) p(x_0,u_0,x_1,u_1,x_2)     \label{eqn:cond_prob}
\end{align}
The last expansion is done using the Bayes Theorem. Apply the Bayes Theorem again, and assume the prior distribution of $p(X)$ is uniform,  we can conclude that the \textit{maximum a posteriori} (MAP) distribution of $X$ follows \cite{dellaert2017factor}
$$
X^{MAP} = \argmax_{X} p(Z|X) = \argmax_{X} l(X;Z)  = \argmax_{X} \phi(X)
$$
where $l(X;Z)$ is the product of likelihood functions obtained by rewriting conditional probability terms in Eq. (\ref{eqn:cond_prob}) to their counterparts in (\ref{eqn:likelihood_x}), (\ref{eqn:likelihood_u}), or (\ref{eqn:likelihood_cst}). $\phi(X)$ is a simplified notation defined as $l(X;Z) = \phi(X) = \prod \phi_i(X_i)$. $\phi_i$ is still the likelihood function we defined earlier, and $X_i$ is a set of elements of $X$ that relates to the function $\phi_i$. We call a $\phi_i$ as a factor.

The key procedure links the probabilistic view of the factor graph and the LQR is the VE. When $X = X^{MAP}$, $\phi(X^{MAP}) \propto p(X^{MAP})$. Let $X = [\theta_0\dots \theta_n]$, we can factorize $p(X)$ as  
\begin{equation}
   p(X) = p(\theta_0|S_0)p(\theta_1|S_1)\dots p(\theta_n) = \prod_{j}p(\theta_j|S_j). \label{eqn:prob_ve}
\end{equation}
The $S_j$ is called \textit{separator} \cite{blair1993introduction}, which is defined as the set of variables that $\theta_j$ is conditioned after the factorization. This factorization process is the VE. Its final form depends on the \textit{elimination order}, which is the order how elements in $X$ got picked during VE. More importantly, in the case of $X$ contains states and control inputs, when control $u_i$ in $X$ is picked, \textbf{the factorized term $p(u_i|S_i)$ is the optimal feedback controller}. 


To better present the detailed steps of VE, we convert the probabilistic view to a matrix view using the fact that our likelihood functions are Gaussian distributions. From Definition (\ref{eqn:likelihood_x}), (\ref{eqn:likelihood_u}), and (\ref{eqn:likelihood_cst}), we can see all likelihood functions or factors $\phi_i(X_i)$ can be written as 
$$
\phi_i(X_i) \propto \exp \Big\{ -\frac{1}{2}\| A_iX_i - b_i\|^2_{\Sigma_i}    \Big\}
$$
Then 
\begin{align}
X^{MAP} & = \argmax_{X} \phi(X) = \argmin_{X} -2\log(\prod \phi_i(X_i)) \nonumber \\
& = \argmin_{X} \sum_i \| A_iX_i - b_i\|^2_{\Sigma_i}  = \argmin_{X} \| AX - b\|^2_{\Sigma}  \label{eqn:Ax=b}
\end{align}
where $A$, $b$ and $\Sigma$ stack all $A_i$, $b_i$, and $\Sigma_i$ together respectively. Then the solution of $X^{MAP}$ is a linear least square problem. A caveat is the covariance matrix in $(\ref{eqn:likelihood_cst})$ is 0 because the system dynamics constraints must be strictly obeyed. So some terms in $\Sigma$ are zero. If we expand the Mahalanobis norm in (\ref{eqn:Ax=b}) and define weight matrix $W=\Sigma^{-1/2}$, we have $(AX - b)^TW(AX - b)$ with some infinite weights. This weighted linear least square system can be solved by the modified Gram-Schmidt algorithm \cite{gulliksson1995modified}.

Using the matrix view, VE has a direct connection to sparse matrix factorization \cite{dellaert2017factor}. If we factorize matrix $A$ in (\ref{eqn:Ax=b}) as $A=QR$ using the modified Gram-Schmidt, where $Q$ is orthonormal and $R$ is upper-triangular. Then 
$$
\min_{X} \| AX - b\|^2_{\Sigma} = \min_{X} Q^T\| AX - b\|^2_{\Sigma} = \min_{X} \| RX - d\|^2_{\Sigma} + \| e\|^2_{\Sigma}
$$
where $d = Q^Tb$. The last term $\| e\|^2_{\Sigma}$ appears as a residual if $R$ have rows with all 0s on the bottom part. Now each block row of $\| RX - d\|^2_{\Sigma}$ corresponds to one term in (\ref{eqn:prob_ve}) because $R$ is upper-triangular. We shall emphasize that the factorization of A can be done by doing the modified Gram-Schmidt on just one column at a time. Since $i$th column of $A$ corresponds to variable $\theta_i$ in $X$, we ``eliminate'' it. Moreover, $A$ is sparse in the optimal control setting, so the elimination can be done very efficiently. This observation leads to the following VE steps to eliminate $\theta_i$:

%A factor graph is a bipartite graph consists of (1) variable nodes (drawn as circles) that represent unknown variables and (2) factor nodes that represent constraints (drawn as squares) or objectives (drawn as dots), connected by edges.
% Figure \ref{fig:lqr_suba} shows the factor graph corresponding to a 3 time-step LQR problem.
%In the factor graph formulation, 
%states and controls are variables (circles), state objectives and control costs are objective factors (dots), and dynamics constraints are constraint factors (squares). Here we define $x_i \in \mathbb{R}^n$, $u_i \in \mathbb{R}^m$, and other matrices in the system dynamics and cost functions to have proper dimensions.

% To solve the LQR problem, we apply the variable elimination (VE) algorithm to the factor graph in Figure \ref{fig:lqr_suba}.
% At a high level, in VE we solve for one variable at a time and propagate any costs/constraints onto the variables it shares a factor with.
% The general VE algorithm is detailed in Section \ref{sec:ecLQR}, but for simplicity we start with a simplified version specific to the LQR formulation.

% We start by eliminating $x_N$.  $x_N$ shares a factor with $u_{N-1}$ and $x_{N-1}$, so we solve for $x_N$ in terms of $u_{N-1}$ and $x_{N-1}$.

%% favorite:
% \begin{align*}
%     \begin{cases}
%         \phi_{x_i}(x_i) = \phi_{u_i}^*(x_i) + x_i^TQx_i & \text{Collect Costs} \\
%         x_i^*(u_{i-1}, x_{i-1}) = Bu_{i-1} + Ax_{i-1} & \text{Solve for optimal $x_i$}\\
%         \phi_{x_i}^*(u_{i-1}, x_{i-1}) = \phi_{x_i}(x_i^*) & \text{Cost assuming optimal $x_i$}
%     \end{cases}
% \end{align*}
% \begin{align*}
%     \begin{cases}
%         \phi_{u_i}(u_i, x_i) = \phi_{x_{i+1}}^*(u_i, x_i) + u_i^TRu_i & \text{Collect Costs} \\
%         u_i^*(x_{i}) = \argmin_{u_i} \phi_{x_{i+1}}^*(u_i, x_i) & \text{Solve for optimal $u_i$} \\
%         \phi_{u_i}^*(x_{i}) = \phi_{u_i}^*(u_i^*, x_i) & \text{Cost assuming optimal $u_i$}
%     \end{cases}
% \end{align*}

% \begin{algorithm}
% \caption{Variable Elimination on the LQR factor graph}
% \For{$s \in x_N, u_{N-1}, x_{N-1}, \ldots, x_1$}{
%     \eIf{$s$ is a state, $x_i$}{
%         % $\phi_{x_i}(x_i) \leftarrow \phi_{u_i}(x_i) + x_i^TQx_i$ \emph{Collect Factors}
%         $x_i^*(u_{i-1}, x_{i-1}) \leftarrow Bu_{i-1} + Ax_{i-1}$
%         $\phi_{x_i}^*(u_{i-1}, x_{i-1}) \leftarrow \phi_{u_i}^*(x_i^*) + x_i^{*T}Qx_i^*$
%     }{
%         $$u_i^*(x_{i}) \leftarrow \argmin_{u_i} \phi_{x_{i+1}}^*(u_i, x_i)$$
%         $\phi_{u_i}^*(x_{i}) \leftarrow \phi_{x_{i+1}}^*(u_i^*, x_i) + u_i^{*T}Ru_i^*$
%     }
% }
% \end{algorithm}
% \begin{center}
% \setlength\tabcolsep{3pt}
% \begin{tabular}{rl}
%     Eliminate $x_i$: & $\begin{aligned}\begin{cases}
%         % $\phi_{x_i}(x_i) \leftarrow \phi_{u_i}(x_i) + x_i^TQx_i$ \emph{Collect Factors}
%         x_i^*(u_{i-1}, x_{i-1}) = Bu_{i-1} + Ax_{i-1} & \text{Solve for x}\\
%         \phi_{x_i}^*(u_{i-1}, x_{i-1}) = \phi_{u_i}^*(x_i^*) + x_i^{*T}Qx_i^* & \text{factor on separator}
%     \end{cases}\end{aligned}$\\[2em]
%     Eliminate $u_i$: & $\begin{aligned}\begin{cases}
%         u_i^*(x_{i}) = \argmin_{u_i} \phi_{x_{i+1}}^*(u_i, x_i) \\
%         \phi_{u_i}^*(x_{i}) = \phi_{x_{i+1}}^*(u_i^*, x_i) + u_i^{*T}Ru_i^*
%     \end{cases}\end{aligned}$
% \end{tabular}
% \end{center}

% We eliminate variables one at a time starting with $x_N$, then $u_{N-1}, x_{N-1}, \ldots, x_1$.  To eliminate a state,
%We use VE to solve the factor graph. We repeatedly select one variable $\theta_i$ (may be any variable: state or control in this problem) with separator $S_i$ defined as all the variables sharing a factor with $\theta_i$, then:
% \renewcommand{\labelenumi}{%
%   {\ifcase\value{enumi}% 0
%   \or\color{red}% 1
%   \or\color{green}% 2
%   \or\color{blue}% 3
%   \else\fi%
%   \arabic{enumi})}%
% }
% \renewcommand{\labelenumi}{
%     \ifcase\value{enumi}% 0
%     \or\textcolor{red}{\arabic{enumi})}% 1
%     %   \or\color{green}% 2
%     %   \or\color{blue}% 3
%     \else
%         \arabic{enumi})
%     \fi
% }
\begin{itemize}
    \item[\textcolor{red}{Step 1.}]  Identify all the factors directly connected to $\theta_i$ (all block rows in $A$ with nonzero elements on block column $i$). We also extract rows' weights from the weight matrix $W$. Block rows with infinite weights are constraint factor $\psi_i(\theta_i, S_i)$, while block rows with finite weight are objective factor $\phi_i(\theta_i, S_i)$. Now all these block rows formulate $\|A_i[\theta_i;S_i]-b_i\|^2_{\Sigma_i}$ We can normalize finite weights to be 1 by multiplying $\Sigma_i^{-1/2}$ on $A_i$ and $b_i$. 
    \item[\textcolor{blue}{Step 2.}] Factorize $[A_i|b_i]$ to $[R_i|d_i]$ using the modified Gram-Schmidt on its first column. In the case of quadratic costs and linear system dynamics constraints, we can treat it as a constrained least square problem and solve manually, as we show in Figure \ref{fig:lqr_VE}.
    %Solve for the optimal value of $\theta_i$ as a function of its separator variables $\theta_i^*=f_i(S_i)$ that satisfies the constraints $c_i(\theta_i, S_i)=0$ and minimizes the objectives $\phi_i(\theta_i, S_i)$.
    \item[\textcolor{green}{Step 3.}]  Output the first block row of $[R_i|d_i]$ as $p(\theta_i|S_i)$. Add the rest blocks of $[R_i|d_i]$ to replace corresponding blocks in $[A_i|b_i]$.

\end{itemize}
We repeat this process until all variables have been eliminated. More details on the VE algorithm are in \cite{dellaert2017factor}. 

==> sections/sec_intro.tex <==
Equality constrained optimal control problems emerge in motion planning problems of various robotics applications. For example, an aerial vehicle restricts its trajectory on a predefined curve; a robot arm polishing an object constrains its end effector position to lie on the surface of the object; a walking legged robot may has equality constraints that supporting feet positions are constant \cite{farshidian2017real}. 
% One general formulation of an equality constrained discrete-time optimal control problem is 
% \begin{subequations}\label{problem1}
% \begin{align}
%     \min_{\textbf{u}} & \ x_N^TQ_fx_N + \sum_{n=0}^{N-1}(x_n^TQx_n+u_n^TRu_n) \label{eqn:eqn_cost}\\
%     \text{s.t. }      & \ x_{n+1} = x_n + f(x_n,u_n)\Delta t \label{eqn:sys_dyn}\\
%                       & \ g(\textbf{x}, \textbf{u}, n_c) = 0, \ \ \forall n_c \in \mathcal{C}. \label{eqn:eqn_cst} 
% \end{align}
% \end{subequations}
% In Problem \ref{problem1}, $\textbf{x} = [x_0, x_1,\dots,x_N]$ is the state trajectory and $\textbf{u} = [u_0, u_1,\dots,u_{N-1}]$ is the control sequence. Eq. (\ref{eqn:sys_dyn}) is the system dynamics. Eq. (\ref{eqn:eqn_cst}) represents an equality constraint for each $n_c$ in an index set $\mathcal{C}$. We first consider the case that $g(\textbf{x}, \textbf{u}, n_c)$ only involves $x_{n_c}$ and $u_{n_c}$, but in more general settings, such as for periodic trajectories, direct registering gaits, or sequential dependencies, a constraint may involve multiple states and control inputs at different time instances. We call such constraints \textit{cross-time-step} constraints.
We want to find their optimal motion trajectories and optimal controllers. 

To formulate a discretized version of an equality constrained optimal control problem, we define a robot's state trajectory as $\textbf{x} = [x_0, x_1,\dots,x_N]$ where N is the trajectory length and its control input sequence as $\textbf{u} = [u_0, u_1,\dots,u_{N-1}]$. A state trajectory $\textbf{x}^*$ and a control sequence $\textbf{u}^*$ are optimal if a cost function $C(\textbf{x}, \textbf{u})$ is minimized 
subject to two types of constraints on $\textbf{x}$ and $\textbf{u}$.
% Moreover, $\textbf{x}$ and $\textbf{u}$ need to satisfy two types of constraint.
First, the system dynamics of the robot is usually modeled as a differential-algebraic equation (DAE) which imposes constraints on consecutive states and a control: 
$x_{n+1} = x_n + f(x_n,u_n) dt$ 
where $dt$ is the time difference between two states. %The system dynamics imposes constraints on consecutive states.
Second, other problem specific requirements may add a set of equality constraints $g_k(\textbf{x}, \textbf{u}) = 0$ to the problem. 

In this paper we focus on the most basic form of such equality constrained optimal control problems as below: 
%To solve Problem \ref{problem1} for the optimal control sequence and the optimal controller, a common approach is differential dynamic programming (DDP) \cite{mayne1973differential} or its simplified version iLQR \cite{li2004iterative} which essentially consist of iteratively solving the linearized problem:
% DDP starts with an initial nominal controller. It first simulates the system dynamics with the nominal controller to get a state trajectory and a control sequence. Then Eq. (\ref{eqn:sys_dyn}) and (\ref{eqn:eqn_cst}) are linearized along the state trajectory, resulting in a linear problem:


In Problem \ref{problem2} the cost function (\ref{eqn:linear_cost}) is quadratic. The system dynamics constraints (\ref{eqn:linear_sys_dyn}) and problem specific equality constraints (\ref{eqn:linear_eqn_cst}) are linear. $\mathcal{C}$ is a set of indices between 1 to N where a constraint applies. We want to find $\textbf{u}^*$, $\textbf{x}^*$, and the optimal feedback controller $u_i^*=\pi(x_i)$. Studying this basic linear problem form is important. For one thing, it directly applies to all linear systems. For another, it also appears in the linearization step of the optimal control for nonlinear systems with nonlinear constraints \cite{mayne1973differential, li2004iterative}. 

\begin{figure}
    \centering
    \resizebox{8cm}{!}{\input{images/tikz/cross_ec_LQR_fg.tikz}}
    % \includegraphics[width=0.8\linewidth]{images/ec_LQR_fg.eps}
    \caption{The factor graph representation of an equality constrained LQR problem with cross-time-step constraints (i.e. in red) for trajectory length $N=3$.  Our approach can efficiently solve problems with cross-time-step constraints while previous dynamic programming approaches \cite{laine2019efficient} cannot.}
    \label{fig:cross-ec-LQR-factor-graph}
\end{figure}

% Solving Problem \ref{problem2} using dynamic programming (DP) is the key step. The solution can be used to update the nominal controller in a gradient descent algorithm. Then DDP iterates with the updated controller.
% The key insight in efficiently solving Problem \ref{problem2} is to use dynamic programming (DP) \cite{}.
% : solve for the cost that will be incurred at and after $x_n$ (as a function of $x_n$) assuming $u_n, \ldots, u_N$ are optimal, and use these ``\costtogo'' functions to derive optimal control laws.
The constraints (\ref{eqn:linear_eqn_cst}) require special attention to solve. Without (\ref{eqn:linear_eqn_cst}), Problem \ref{problem2} is a standard Linear Quadratic Regular (LQR) problem. It can be solved by constructing the value function (\costtogo{}) using the Ricatti equations in a backward pass \cite{bertsekas1995dynamic}. This method is based on dynamic programming (DP). The computational complexity of this DP approach grows linearly with the trajectory length. When constraints (\ref{eqn:linear_eqn_cst}) are present, \cite{laine2019efficient} proposes the construction of \constrainttogo{} in order to generalize the DP step to equality constrained LQR. At each time $t$ during the DP backward pass, the optimal controller should minimize a cost function subject to a constraint which includes a term from the \constrainttogo{}, representing the constraints on $x_t$ due to future constraints.

% However, with the constraints (\ref{eqn:linear_eqn_cst}) in the problem, the \costtogo{} is no longer sufficient to capture the additional constraints on the variables.  General approaches for solving constrained least squares problems, such as solving the KKT conditions directly, can be used, but these scale in computational complexity with the cube of trajectory length.  Recently, \cite{laine2019efficient} showed how to achieve linear complexity by constructing the \constrainttogo{} in addition to the \costtogo{}.  However, \cite{laine2019efficient} only addresses constraints within the same time-step and cannot natively handle cross-time-step constraints.

% However, with the constraints (\ref{eqn:linear_eqn_cst}) in the problem, the \costtogo{} is no longer sufficient to capture the additional constraints on the variables.
% Specifically, $x_n$ may have some obscure constraints if the allowable actions of $u_n$ are insufficient to satisfy constraints on $x_{n+1}$ for any choice of $x_n$.
% One na\"ive approach to deal with the constraints (\ref{eqn:linear_eqn_cst}) is use Lagrange multipliers to construct an unconstrained problem then solve the KKT conditions for this new problem \cite{sideris2011riccati}.
% % With constraint (\ref{eqn:linear_eqn_cst}) in the problem, state and control must strictly obey the constraint equations. If no equality constraint present, Problem \ref{problem2} is normal LQR. We can construct value function (or \textit{cost-to-go}) and solve Riccati equations backwards to get the optimal controller \cite{bertsekas1995dynamic}. The computational complexity of DP grows linearly with the trajectory length $N$. With the constraints, we can use Lagrangian multiplier to construct an unconstrained problem, and then solve KKT conditions for this new problem \cite{sideris2011riccati}.
% However the computational complexity of this method has cubic relationship to the trajectory length. In order to apply DP, a key contribution of \cite{laine2019efficient} is constructing a \textit{constraint-to-go} function as an additional constraint that the current control needs to satisfy. The \textit{constraint-to-go} is updated during DP steps along with the \textit{cost-to-go}.
% %%%%% this is a statement I am not quite confident
% However, \cite{laine2019efficient} can only handle constraints where all variables are at the same time step, and solving problems with constraints on variables at multiple time-steps (e.g. $u_1+u_2+u_3 = 1$) would require adding record-keeping state dimensions or similarly unpleasant reformulations.
% % However, this method only works for constraints that contain state and control variables at the same time step. It is not possible to deal with cross-time-step constraints.

Notice from (\ref{eqn:linear_eqn_cst}) that we first consider the case that one $g_k(\textbf{x}, \textbf{u})$ only involves $x_{n_c}$ and $u_{n_c}$ at the same time step $n_c$, but in more general settings, a constraint may involve multiple states and control inputs at different time instances. We call such constraints \textit{cross-time-step} constraints. They may appear in a number of problems such as for generating periodic gaits or operating under complex control limits.  As an example, consider a case where we seek to generate a periodic quadruped gait with fixed stride length.  The absolute contact locations for each foot may be anywhere, but the relative distance between two contacts is fixed.  Then the constraint for the second foot may look like 
% $\begin{bmatrix}I&0&0&0\end{bmatrix}x_{25} - \begin{bmatrix}I&0&0&0\end{bmatrix}x_5 = d$
$[0~I~0~0]x_{25} - [0~I~0~0]x_5 = 30cm$.  As another example, consider a case where the total motor torque while in ground contact is fixed due to power system limits.  Then the constraint may look like $u_5+\ldots+u_{10} = 5Nm$.

In this paper we propose a novel formulation using factor graphs \cite{cunningham2010ddf} to solve general linear equality constrained linear optimal control problems. The equality constraints can relate any states and/or controls at any time instances. We use a factor graph to represent the problem,
% In the graph, the cost function is Gaussian factors; the system dynamics are hard constraint factors; the equality constraints are also hard constraint factors.
and use Variable Elimination (VE) on the factor graph \cite{dellaert2017factor} to solve for
optimal trajectories and optimal controllers.
% An advantage of our approach over traditional methods is the ability to handle cross-time-step constraints. 
%To deal with conflicting constraints, we develop \textit{double QR} algorithm to replace conventional QR factorization during variable elimination.
As long as the maximum number of variables involved in all constraints is bounded, the computational complexity of our method grows linearly with the trajectory length.
We match state of the art complexity \cite{laine2019efficient}, even for the more general cross-time-step constraints which \cite{laine2019efficient} does not handle.

Our contributions are:
\begin{itemize}
    \item We propose using factor graphs as a novel representation for equality constrained optimal control problems. We claim this representation is more flexible and intuitive
    % than traditional equation or matrix representations,
    which allows it to handle more general constraints than existing methods.
    \item We present how VE on the factor graph representation can efficiently derive the \textit{cost\_to\_go} function, the \textit{constraint\_to\_go} function, and the optimal controller at each time step for equality constrained LQR problems.
\end{itemize}

==> sections/sec_method_constrainedopt.tex <==
% \subsubsection*{Methods for Variable Elimination}
\green{Step 2} of the variable elimination algorithm involves solving the constrained optimization problem
\begin{align}
    x_i^* = \argmin_{x_i} \phi_i(x_i, S_i) \quad \suchthat c_i(x_i) = 0 \label{eq:VE_argmin}
\end{align}
\textit{This can be solved using any number of methods and VE is agnostic to which method is used.}  In the case of equality constrained LQR, $\phi_i$ takes a positive semi-definite quadratic form and $c_i$ takes a linear form making (\ref{eq:VE_argmin}) equivalent to a constrained least squares problem which can be solved using e.g. a modified QR factorization, directly solving the KKT matrix, or SVD as in \cite{laine2019efficient}. Moreover, for linear problem with invertible or full column rank constraint matrices, the optimal solution is unique. 

We will now briefly describe the modified QR factorization technique. The modified QR factorization technique that handles linear constraints reformulates constraints as rows which are weighted infinitely heavily, and the modified QR can be performed with a modified Gram-Schmidt process.  We create the least squares matrix such that the top $n_c$ rows represent the constraint equations (and have infinite weight) and the remaining $n_\phi$ rows represent the optimization objective.  Then, we perform $n_c$ iterations of Gauss-Jordan Elimination using the top $n_c$ rows, followed by standard QR using Gram-Schmidt \cite{gander1980algorithms} on the bottom rows.  Intuitively, row reduction represents direct substitution with naturally corresponds to enforcing an equality constraint.  More formally, it can also be shown that the normalization step in Gram-Schmidt will behave exactly like row reduction when there exists a non-zero entry with zero covariance in column $j$.  See \cite{gulliksson1995modified} for a rigorous derivation of constrained least squares using Gram-Schmidt, especially Eq. (2.8).
% 
% \subsection{Hard Constraints In Variable Elimination}\label{sec:hard_constraint}
%     In our LQR formulation, we made use of so called ``hard constraints'', but handling hard constraints requires special attention. Naively representing hard constraints as zero-covariance distributions as written in Eq. (\ref{eq:lqr_hardconstraint}) will result in infinite entries in rows of $A_i$.  
%     %\cite{ta2014factor} mentions a Gram-Schmidt process to perform QR factorization even with 0 covariance rows but doesn't specify how this is done.  We will briefly describe how.
% 
    % To deal with this problem, we use a modified version of the standard algorithm for QR using Gram-Schmidt \cite{gander1980algorithms} to essentially perform a row reduction for constraint rows and standard column-wise Gram-Schmidt otherwise.  More precisely, to factor the matrix with covariance $A, \sigma_A$ into $QR$ with covariance $\sigma_R$, we iterate column-wise following the usual Gram-Schmidt process.  If a column $A_{*, j}$ contains a non-zero entry $A_{i, j}$ on a constraint row $i$, we simply copy $R_{j, *} \leftarrow A_{i, *}$ and $\sigma_{R_i} \leftarrow \sigma_{A_i}$ then perform row reduction $A \leftarrow A - A_{*, j}A_{i,*}$, where $*$ denotes the entire row/column (note that the constraint row $A_{i, *}$ will get zeroed out).  Otherwise, perform Gram-Schmidt for QR as usual \cite{gander1980algorithms}.
    % 
    % Intuitively, row reduction is a natural step to perform for constraints since row reduction represents direct substitution.  More formally, it can also be shown that the normalization step in Gram-Schmidt will behave exactly like row reduction when there exists a non-zero entry with zero covariance in column $j$.  See \cite{gulliksson1995modified} for a rigorous derivation of constrained least squares using Gram-Schmidt, especially Eq. (2.8).
    % 
    %         
    % What's more, applying VE with elimination ordering $x_N, u_{N-1}, x_{N-1}, \ldots, x_1$ results in the exact same algorithm as the dynamic Ricatti equation, which is derived by calculating the value function for each state in a backward pass and using $P_n$ with $R$ to find the optimal policy $u^*=-Kx$.  To illustrate this, consider the first two iterations of VE in Figures \ref{fig:lqr_subb} and \ref{fig:lqr_subc}.  $x_2$ is eliminated in \ref{fig:lqr_subb} resulting in an expression for $x_2$ as a function of $x_1$ and $u_1$, as well as a cost that \textit{will} be incurred on $x_2$ as a function of $x_1$ and $u_1$.  In \ref{fig:lqr_subc}, $u_1$ is eliminated resulting in an expression for the optimal $u_1$ in terms of $x_1$, as well as \textit{the total cost that will be incurred in the future assuming optimal control} as a function of $x_1$: $x_1^TP_1x_1$ which is exactly the value function.  Continuing in this fashion, the ``new factors'' $\tau(S(x_n))$ will represent the costs for future timesteps given the current state (which make up the separator $S$), and the conditionals $p(u_n | S(u_n))$ will represent the optimal control laws for the current control given the current state.  Note also that each iteration of variable elimination is essentially solving a constrained least squares problem of just 2 or 3 variables -- the same as in the dynamic Ricatti equation.  For a more comprehensive mathematical derivation of equivalence, please refer to \cite{gerryyetong2019lqrfg}.
% 
    % We can modify the standard algorithm for QR using Gram-Schmidt \cite{gander1980algorithms} to keep track row covariances and leave constraint rows in their non-whitened forms.  Then the $i^{th}$ row of $A$ can be represented as a pair $(\sigma_i, A_i)$.  In the $j^{th}$ iteration of standard Gram-Schmidt for QR, we take the column, $^jA$, of A and set
    % \begin{align*}
    %     ^jQ ~&\leftarrow ~^jA / ||^jA|| \\
    %     R_{i, k} ~&\leftarrow~ ^jA \cdot ^kQ \\
    %     ^kA ~\leftarrow~ ^kA - R_{i, k} ~^kQ
    % \end{align*}
    % for $k=j\ldots n$.  In our modified Gram-Schmidt for QR, 
    % 
    % Finally, we note the powerful statement that, although we have demonstrated using Gram-Schmidt for VE with constraints, VE for the factor graph formulation of LQR is indifferent to how the factorization in \ref{eq:prelim_VE_factorize} is computed.  Any method for solving constrained least squares problems followed by appropriate back-substitution can be used in place of Gram-Schmidt, such as SVD as used by \cite{laine2019efficient} or a 2-step substitution-optimization scheme (although we will see later that Gram-Schmidt has better theoretical complexity than SVD).  \textit{Because VE defines the sparsity pattern rather than the underlying implementation, we propose that VE on factor graphs is a useful abstraction for solving general optimal control problems.}


==> sections/sec_preliminary.tex <==
In this section we present a factor graph formulation from \cite{gerryyetong2019lqrfg} for the LQR problem which results in a solution equivalent to the common Ricatti solution, briefly summarize the VE algorithm for optimizing factor graphs,  and describe how to handle ``hard constraints'' in factor graphs.
%which are needed for the LQR problem formulation.
\subsection{LQR as a Factor Graph} \label{sec:prelim_LQR}
    A factor graph is a probabilistic graphical model which represents a  joint probability distribution over variables into a product of factors, each involving a subset of the variables in the joint distribution.  Graphically, we depict a factor graph as in Figure \ref{fig:ec-LQR-factor-graph} where variables (circles) are connected via edges to factors (dots and squares).
    Expressing joint distributions as a product of factors allows us to exploit sparsity structure in problems that arises from domain expertise to solve problems more efficiently.
    
    We can express the LQR problem in a factor graph by considering that minimizing a sum of quadratic costs is equivalent to minimizing the negative log likelihood of a product of Gaussians.  As an example, we can consider the cost function for a single time step from Eq. (\ref{eqn:eqn_cost}):
    % The equivalence of maximizing a multivariate Gaussian distribution and performing least squares is central to the formulation of LQR as a factor graph, since minimizing the sum of quadratic state and control costs can be equivalently expressed as maximizing a product of Gaussian distributions whose means are desired values and whose information matrices (inverse of variance matrix) are the quadratic cost matrices, $Q$ and $R$ from Equation \ref{eqn:eqn_cost}:
    \begin{align*}
        x^TQx + u^TRu = -\log p(x, u) + c
        % \text{for } p(x, u) \propto \exp{\left(-\frac{1}{2}\left(\frac{x-\mu_x}{\sigma_x}\right)^2\right)}
        % \exp{\left(-\frac{1}{2}\left(\frac{u-\mu_x}{\sigma_u}\right)^2\right)}
    \end{align*}
    
    for $p(x, u) \propto \exp{(-\frac{1}{2}(\frac{x-\mu_x}{\sigma_x})^2)}
    \cdot \exp{(-\frac{1}{2}(\frac{u-\mu_u}{\sigma_u})^2)}$ \\[0.5em]
    where $\mu_x = 0$, $\mu_u = 0$, $\sigma_x^{-2}=Q$, $\sigma_u^{-2} = R$, and $c$ is some normalizing constant.Thus, each quadratic cost corresponds to one Gaussian factor (``soft objective'').  
    
    Furthermore, we can represent a dynamics equation as a ``hard constraint'' factor, or a distribution with 0 covariance:  
    \begin{align}
        x_{n+1} &= x_n + f(x_n, u_n)\Delta t \nonumber\\ &\implies
        \exp({\scriptstyle-\frac{1}{2} \left(\frac{ -x_{n+1} + x_n + f(x_n, u_n)\Delta t }{\sigma}\right)^2}) \label{eq:lqr_hardconstraint}
    \end{align}
    where $\sigma\to 0$. Satisfying this constraint means minimizing the negative log likelihood of this distribution.

    \begin{figure}
        \centering
        \begin{subfigure}[t]{0.9\linewidth}
            \centering
            \includegraphics[width=.9\textwidth]{images/varElim/varElim_1.eps}
            \caption{}
            \label{fig:lqr_suba}
        \end{subfigure}
        \begin{subfigure}[t]{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{images/varElim/varElim_2.eps}
            \caption{}
            \label{fig:lqr_subb}
        \end{subfigure}
        \begin{subfigure}[t]{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{images/varElim/varElim_3.eps}
            \caption{}
            \label{fig:lqr_subc}
        \end{subfigure}
        \caption{Factor graph of an LQR problem (a) before elimination, (b) after eliminating $x_2$, and (c) after eliminating $u_1$}
        \label{fig:lqr}
        % TODO(gerry): use Q_f on final time step and also resize screenshots better
    \end{figure}
    
    Putting together the negative log likelihood form of all factors, Figure \ref{fig:lqr_suba} depicts the factor graph formulation of a LQR problem with trajectory length 3.  
    %Because constrained least squares is equivalent to maximizing a product of soft objectives and hard constraints, it follows that 
    %Optimizing the factor graph will give the solution to the LQR problem.


\subsection{Variable Elimination on Factor Graphs}
    The VE algorithm finds variable assignments which minimize the negative log likelihood by solving one variable at a time.  At each iteration, all factors, $\phi_j(x_i, \ldots)$, connected to variable $x_i$ are collected into a single factor, $\psi_i(x_i, S_i) \coloneqq \prod \phi_j(x_i, \ldots)$, which is factored into a conditional probability, $p(x_i | S_i)$, and a new factor, $\tau(S_i)$, on the separator, $S_i$ (the separator is defined as all variables sharing a factor with $x_i$):
    \begin{align}
        \phi(x_i, \ldots, x_n)
            &= \psi_i(x_i, S_i) \cdot \phi(x_{i+1}, \ldots, x_n) \nonumber \\
            &= p(x_i | S_i) \cdot \tau(S_i) \cdot \phi(x_{i+1}, \ldots, x_n) \label{eq:prelim_VE_factorize}
    \end{align}
    
    Intuitively, we can interpret one iteration of the variable elimination algorithm as factoring a total cost $\psi_i(x_i, S_i)$ into \begin{description}
        \item[$p(x_i|S_i)$:] a distribution which essentially tells us the optimal $x_i$ given the variables sharing a factor with it, and \item[$\tau(S_i)$:] the negative log likelihood on the remaining variables sharing a factor with $x_i$, assuming $x_i$ is optimal.
    \end{description}
    
    As the negative log likelihood of factors can be written in matrix form, Eq. (\ref{eq:prelim_VE_factorize}) is solved using QR factorization:
    \begin{align} \label{eqn:elimination}
        \min ||A_i[x_i; S_i]||^2_{\Sigma} &= ||R_ix_i + T_iS_i||^2 + ||A_\tau S_i||^2
    \end{align}
    where $A_i=Q\begin{bmatrix}R_i & T_i \\ &A_\tau\end{bmatrix}$ is the QR factorization of $A_i$ \cite{dellaert2017factor}. The two terms on the right hand side corresponds to $p(x_i | S_i)$ and $\tau(S_i)$.
    For additional background on factor graphs and VE, we defer to \cite{dellaert2017factor}.
    

\subsection{Hard Constraints In Variable Elimination}\label{sec:hard_constraint}
    In our LQR formulation, we made use of so called ``hard constraints'', but handling hard constraints requires special attention. Naively representing hard constraints as zero-covariance distributions as written in Eq. (\ref{eq:lqr_hardconstraint}) will result in infinite entries in rows of $A_i$.  
    %\cite{ta2014factor} mentions a Gram-Schmidt process to perform QR factorization even with 0 covariance rows but doesn't specify how this is done.  We will briefly describe how.

    To deal with this problem, we use a modified version of the standard algorithm for QR using Gram-Schmidt \cite{gander1980algorithms} to essentially perform a row reduction for constraint rows and standard column-wise Gram-Schmidt otherwise.  More precisely, to factor the matrix with covariance $A, \sigma_A$ into $QR$ with covariance $\sigma_R$, we iterate column-wise following the usual Gram-Schmidt process.  If a column $A_{*, j}$ contains a non-zero entry $A_{i, j}$ on a constraint row $i$, we simply copy $R_{j, *} \leftarrow A_{i, *}$ and $\sigma_{R_i} \leftarrow \sigma_{A_i}$ then perform row reduction $A \leftarrow A - A_{*, j}A_{i,*}$, where $*$ denotes the entire row/column (note that the constraint row $A_{i, *}$ will get zeroed out).  Otherwise, perform Gram-Schmidt for QR as usual \cite{gander1980algorithms}.
    
    Intuitively, row reduction is a natural step to perform for constraints since row reduction represents direct substitution.  More formally, it can also be shown that the normalization step in Gram-Schmidt will behave exactly like row reduction when there exists a non-zero entry with zero covariance in column $j$.  See \cite{gulliksson1995modified} for a rigorous derivation of constrained least squares using Gram-Schmidt, especially Eq. (2.8).
    
            
    What's more, applying VE with elimination ordering $x_N, u_{N-1}, x_{N-1}, \ldots, x_1$ results in the exact same algorithm as the dynamic Ricatti equation, which is derived by calculating the value function for each state in a backward pass and using $P_n$ with $R$ to find the optimal policy $u^*=-Kx$.  To illustrate this, consider the first two iterations of VE in Figures \ref{fig:lqr_subb} and \ref{fig:lqr_subc}.  $x_2$ is eliminated in \ref{fig:lqr_subb} resulting in an expression for $x_2$ as a function of $x_1$ and $u_1$, as well as a cost that \textit{will} be incurred on $x_2$ as a function of $x_1$ and $u_1$.  In \ref{fig:lqr_subc}, $u_1$ is eliminated resulting in an expression for the optimal $u_1$ in terms of $x_1$, as well as \textit{the total cost that will be incurred in the future assuming optimal control} as a function of $x_1$: $x_1^TP_1x_1$ which is exactly the value function.  Continuing in this fashion, the ``new factors'' $\tau(S(x_n))$ will represent the costs for future timesteps given the current state (which make up the separator $S$), and the conditionals $p(u_n | S(u_n))$ will represent the optimal control laws for the current control given the current state.  Note also that each iteration of variable elimination is essentially solving a constrained least squares problem of just 2 or 3 variables -- the same as in the dynamic Ricatti equation.  For a more comprehensive mathematical derivation of equivalence, please refer to \cite{gerryyetong2019lqrfg}.

    % We can modify the standard algorithm for QR using Gram-Schmidt \cite{gander1980algorithms} to keep track row covariances and leave constraint rows in their non-whitened forms.  Then the $i^{th}$ row of $A$ can be represented as a pair $(\sigma_i, A_i)$.  In the $j^{th}$ iteration of standard Gram-Schmidt for QR, we take the column, $^jA$, of A and set
    % \begin{align*}
    %     ^jQ ~&\leftarrow ~^jA / ||^jA|| \\
    %     R_{i, k} ~&\leftarrow~ ^jA \cdot ^kQ \\
    %     ^kA ~\leftarrow~ ^kA - R_{i, k} ~^kQ
    % \end{align*}
    % for $k=j\ldots n$.  In our modified Gram-Schmidt for QR, 
    
    Finally, we note the powerful statement that, although we have demonstrated using Gram-Schmidt for VE with constraints, VE for the factor graph formulation of LQR is indifferent to how the factorization in \ref{eq:prelim_VE_factorize} is computed.  Any method for solving constrained least squares problems followed by appropriate back-substitution can be used in place of Gram-Schmidt, such as SVD as used by \cite{laine2019efficient} or a 2-step substitution-optimization scheme (although we will see later that Gram-Schmidt has better theoretical complexity than SVD).  \textit{Because VE defines the sparsity pattern rather than the underlying implementation, we propose that VE on factor graphs is a useful abstraction for solving general optimal control problems.}
